Solving linear programs on factorized databases

A typical workflow for solving a linear programming problem is to first write a linear program parametrized by the data in a language such as Math GNU Prog or AMPL then call the solver on this program while providing the data. When the data is extracted using a query on a database, this approach ignores the underlying structure of the answer set which may result in a blow-up of the size of the linear program if the answer set is big. In this paper, we study the problem of solving linear programming problems whose variables are the answers to a conjunctive query. We show that one can exploit the structure of the query to rewrite the linear program so that its size depends only on the size of the database and not on the size of the answer set. More precisely, we give a generic way of rewriting a linear program whose variables are the tuples in Q(D) for a conjunctive query Q and a database D into a linear program having a number of variables that only depends on the size of a factorized representation of Q(D), which can be much smaller when the fractional hypertree width of Q is bounded.

==> DWC.tex <==
%auto-ignore
In this section, we formalize the main problem we are solving in this paper, the
{\em dependency weighted counting} problem and give basic observations on its
complexity. 
%

\begin{definition}
  Let $S$ be a relation with attributes $\varx$ and domain $D$, that is, $S
  \subseteq D^\varx$. A \emph{weighting for $S$} is a function
    $\om:S\to \R_+$. A \emph{dependency weighting for $S$} is a weighting for
    $S$ that satisfies $\sum_{\{\tau \in S \mid \tau(x)=d\}} \om(\tau) \le 1$
    for all attributes $x\in\varx$ and database elements $d \in \dom$. The
  \emph{dependency weighted count} of $S$, denoted as $\DWC(S)$, is the maximal
  value of $\sum_{\tau\in S} \om(\tau)$ where the maximum is taken over every
  dependency weighting $\om$ of $S$.
\end{definition}

In the definition of dependency weightings and in rest of the paper, 
we will often refer to the subset of tuples of $S$
whose value on an attribute $x$ equals $d$. We will denote this set as
$\tupleset{x}{d} := \{\tau \in S \mid \tau(x) = d\}.$
Intuitively, $\DWC(S)$ measures the statistical quality of the 
sample $S$, considering that any two database tuples in 
$\tupleset{x}{d}$ are not independent, given that they share the value $d$
on attribute $x\in X$. Therefore, the weights of the 
dependent tuples in $\tupleset{x}{d}$ are constrained
to sum up to at most $1$.


\begin{example}
  Consider the database domain $D=\{0,1\}$, the set of attributes $\{x, y, z\}$
  and the relation
\begin{center}
\begin{tabular}{|c|c|c||c|}\hline
$x$ & $y$ & $z$  &\text{tuple} \\ \hline\hline
$1$ & $1$ & $0$ & $\tau_0$      \\ \hline
$1$ & $0$ & $1$ & $\tau_1$      \\ \hline
$0$ & $1$ & $1$ & $\tau_2$      \\ \hline
\end{tabular}
\end{center}

The set of linear constraints that any dependency weighting $\om:S\to
\R_+$ %\janfoot{the term ``dependency weighting'' was not defined,
      %only the notation $\om$ was locally introduced in some
      %subsubphrase in the definition above and is now out of scope
      %(as the definition didn't assert the notation $\om$ has a
      %global meaning).} 
must satisfy is the following:
$$
\begin{array}{cl@{\qquad}cl}
\val{\om}{\tau_2}  \leq 1 &\text{($\tupleset{x}{0}$)}&
\val{\om}{\tau_0} + \val{\om}{\tau_1}  \leq 1 &\text{($\tupleset{x}{1}$)}\\
\val{\om}{\tau_1}  \leq 1 &\text{($\tupleset{y}{0}$)}&
\val{\om}{\tau_0} + \val{\om}{\tau_2}  \leq 1 &\text{($\tupleset{y}{1}$)}\\
\val{\om}{\tau_0}  \leq 1 &\text{($\tupleset{z}{0}$)}&
\val{\om}{\tau_1} + \val{\om}{\tau_2}  \leq 1 &\text{($\tupleset{z}{1}$)}
\end{array}
$$
For this example, $\DWC(S) = 1.5$, obtained by taking the dependency weighting
$\om:S\to \R_+$ defined as $\val{\om}{\tau} = 0.5$ for all $\tau\in S$. \qed
\end{example}\label{ex:1}

We can define the $\DWC(S)$ equivalently by the following 
linear program $\nlp{S}$ 
whose variables are the database tuples in $S$:
$$
\begin{gathered}
    \text{max } \sum_{\tau \in S} \tau  \text{ subject to } \bigwedge_{\tau \in S} 0 \le \tau \wedge \bigwedge\limits_{x\in X}\bigwedge\limits_{d\in D} \sum_{\tau \in \tupleset{x}{d}} \tau \le 1
\end{gathered}
$$
The positivity constraint $0 \le \tau$ is syntactic sugar for
the inequality $(-1)\tau\le 0$. It should be obvious that the
optimal value of $\nlp{S}$ is equal to 
$\DWC(S)$. 

\begin{example}\label{ex:2}
The linear program $\nlp{S}$ for the set of database tuples
from Example \ref{ex:1} is:
$$
\ max\ \tau_0+ \tau_1+\tau_2\ 
subject\ to \ \left(
\begin{array}{c}
0\le \tau_0 \wedge \tau_2\leq 1   \wedge
\tau_0+\tau_1  \leq 1 \wedge \\
0\le \tau_1 \wedge \tau_1 \leq 1 \wedge
\tau_0 + \tau_2  \leq 1 \wedge\\
0\le \tau_2 \wedge \tau_0  \leq 1  \wedge
\tau_1 + \tau_2  \leq 1 \ \
\end{array} \right) \ \qed
$$

\end{example}

\reviewer{1}{The notation used is a bit odd. For one thing, you are using a tuple $\tau$ to refer to the corresponding variable $\omega(\tau)$ in the linear program, which involves some notation abuse but is still acceptable.} 
\todo{Clarify the notation}

A set $S$ of database tuples may be specified in many different ways, for
instance by the answer set of a database query, by an explicit list, or by a
{\ddcircuit}. The complexity of $\DWC$ thus depends on the way $S$ is given in
the input.

% \begin{definition}[Descriptor classes for sets of database tuples]
% A descriptor class $\DESC=(\Desc,\Vars,\DOM,\SET)$ such that 
% $\Desc$ is a set of descriptors, such that for any $\desc\in \Desc$, 
% $\Vars(\desc)$ and $\DOM(\desc)$ are finite sets and $\SET(\desc)$
% is  set of database tuples with attributes in $\Vars(\desc)$ and 
% database elements $\DOM(\desc)$.
% \end{definition}

% \begin{definition}[Dependency weighted counting problem]
% Given a descriptor class $\DESC=(\Desc,\Vars,\DOM,\SET)$ for sets 
% of database tuples, $\DWC_\DESC$ is the computational problem that inputs a 
% descriptor $\desc\in \Desc$ and 
% outputs $\DWC(\SET(\desc))$.
% \end{definition}

% The complexity of solving $\DWC_\DESC$ depends on the choice of
% parameter $\DESC$, i.e., on the way in which sets of database tuples are
% described.
If $S$ is given explicitly as a list, then it is easy to see that the problem
can be solved in polynomial time, since then $\nlp{S}$ is of size
$O(|X||D||S|)$. That is, $\nlp{S}$ is of size polynomial in the input and one
just has to solve the linear program in polynomial time. However, if $S$ is
specified as the answer set of a query $Q$ on a database $\db$, it may be too
costly to compute it explicitly and then solve $\nlp{S}$ as $S$ may be of
exponential size. Unfortunately, it turns out that solving $\DWC$ when $S$ is
given as a conjunctive query on a database is not tractable. 

% A more interesting descriptor class is $\CQ$ whose descriptors
% $\desc=(Q,D)$ consist of a conjunctive query $Q$ and a 
% relational structure $D$ over the same relational signature, such that $\Vars(\desc)$ 
% is the set of free variables of $Q$, $\DOM(\desc)$ is the domain of
% relational structure $D$, and $\SET(\desc)$ the answers
% set of the conjunctive query $Q$ and the database $D$.


% We introduce the decision problem $\dwacqdec$ associated with $\DWC_{CQ}$ that takes a pair $(Q, D)$ as
% input and outputs the truth-value of $\DWC(\SET(Q, D))$.
% We also introduce the decision problem CQ-SAT that takes a pair $(Q, D)$ as input and outputs the
% truth-value of $\SET(Q, D) = \emptyset$. We will show that these two problems are equivalent using the 
% following lemma.
\begin{lemma}
	\label{lem:equivProblems}
  The problem of deciding on input $(Q,\db)$ whether $\DWC(Q(\db)) > 0$ is $\NP$-hard, where $Q$ is a conjunctive query
  and $\db$ a database.  
\end{lemma}

\begin{proof}
  We show this lemma by showing that $\DWC(Q(\db)) > 0 \Leftrightarrow Q(\db)
  \neq \emptyset$. The $\NP$-hardness then follows since it is known that
  deciding whether the answer set of a conjunctive query is non-empty is
  $\NP$-hard for combined complexity~\cite{chandra77}.

  We start by showing that if $Q(\db) \neq \emptyset$ then $\DWC(Q(\db))>0$. Let
  $\tau \in Q(\db)$. Let $\om$ be the tuple weighting such that $\om(\tau)=1$
  and $\om(\tau') = 0$ for every $\tau' \in Q(\db)$ with $\tau' \neq \tau$. It
  is easy to check $\tau$ is a dependency weighting of $Q(\db)$, thus,
  $\DWC(Q(\db)) \geq 1 > 0$.

  Now assume that $\DWC(Q(\db)) = s > 0$. That is, there exists a weighting
  $\om$ of $Q(\db)$ such that $\sum_{\tau \in Q(\db)} \om(\tau) = s$. If $Q(\db)
  = \emptyset$, this would imply $\sum_{\tau \in Q(\db)} \om(\tau) = 0$, a
  contradiction.
  
	% \begin{itemize}
	% 	\item if $\SET(Q, D) = \emptyset$ then $\nlp{\SET(Q, D)}$ has no variables and its objective 
  %       function is the empty sum so its value is necessarily 0 thus 
  %       \textbf{$\SET(Q, D) = \emptyset \Rightarrow \DWA(\SET(Q, D)) = 0$}		
  %       \item if $\SET(Q, D) \neq \emptyset$. Let $\alpha \in \SET(Q, D)$, we set $W_\alpha = 1$. 
  %           For all $\beta \in \SET(Q, D)$ such that $\beta \neq \alpha$, we set $W_\beta = 0$. 
  %           It is a solution as every sum of variables that could 
	% 		appear in a constraint is either 0 or 1. The objective function of the linear program 
  %           equals 1 for this solution so we can infer that 
  %           $\SET(Q, D) \neq \emptyset \Rightarrow \DWA(\SET(Q, D)) \neq 0$ 
	% 		thus \textbf{$\DWC(\SET(Q, D)) = 0 \Rightarrow \SET(Q, D) = \emptyset$} 
  %           by contraposition.
	% \end{itemize}
\end{proof}

% We can easily conclude from this lemma that CQ-SAT is reducible to $\dwacqdec$. 
% It is well known that CQ-SAT is NP-complete \cite{chandra77} so $\dwacqdec$
% is NP-hard for an arbitrary conjunctive query.

When $S$ is given as a {\ddcircuit} however, the $\DWC$ problem
can be solved in polynomial time. This is the main result of this paper.

\subsection{A tractable algorithm for DWC}

\begin{theorem}
  \label{thm:fr-tractable} Given a {\ddcircuit} $\circuit$, one can compute
  $\DWC(\solcircuit{})$ in time polynomial in the size of $\circuit$.
\end{theorem}

We define a linear program $\clp{\circuit}$ on the edges of $\circuit$ which we claim to be 
equivalent to $\nlp{\solcircuit{}}$. We assume wlog that the root $r$ of $\circuit$ has a single 
ingoing edge which we call the \emph{output edge} $\rootedge$. 

\begin{definition}[$\clp{\circuit}$]

    max  $\rootedge$ 
    s.t. 
    $\bigwedge\limits_{u \in \orsym-gates{\circuit}}$

\end{definition}

Observe that given a circuit $\circuit$, $\clp{\circuit}$ is linear in the size of $\circuit$ 
and that it is straightforward to generate it in linear time. We thus propose the following 
tractable algorithm to compute $\DWC(\solcircuit{})$.

\begin{lstlisting}[]
Function ComputeDWC(circuit)
    LP  := GenerateLP(circuit)
    DWC := SolveLP(LP)
    Return DWC
EndFunction
\end{lstlisting}

As a corollary of Theorem~\ref{thm:fr-tractable} and Theorem~\ref{thm:cq-to-fr},
we get that for every $k \in \mathbb{N}$, computing $\DWC(Q(\db))$ is tractable
for the class of all conjunctive queries of fractional hypertree width $k$.

\reviewer{4}{Please state the exact complexity of solving the LP DWC over a factorized database. Ideally, please give the combined complexity.}

We do not give complexity bounds in Theorem~\ref{thm:fr-tractable} as we will
see that it mainly depends on a call to an external linear program solver. Our
algorithm roughly works as follows: we show in Section~\ref{sec:weight-corr}
that any weighting on the tuples of $\solcircuit{}$ can be naturally represented as a
weighting of the edges of $\circuit$. We then show in
Section~\ref{sec:applications} how to use this correspondence to rewrite $\nlptext$
into an equivalent polynomial size linear program on the edges of $\circuit$
that we can then solve by calling an external linear program solver.


==> related.tex <==
%auto-ignore

\paragraph{Pattern frequencies and s-measure.}
Evaluating the frequency of a pattern in a graph database is a central task in
data mining. A naive way of evaluating this frequency is to use the number of
matchings of the pattern as a frequency measure. The most important drawback of
this approach is the fact that this measure is not anti-monotone, meaning that a
subpattern may be counter-intuitively less frequent than the pattern itself. A
simple illustration of this phenomenon is when the data graph is a $k$-clique
and we consider the triangle as a pattern and a single edge as a subpattern of
the triangle. Using the number of occurrences as a frequency measure, we realize
that the $k$-clique contains $k \choose 2$ edges and ${k \choose 3} \geq {k
\choose 2}$ triangles. This is because many triangles share common edges. In
many applications, it seems abusive to consider two triangles having a common
edge as two distinct occurrences of the same pattern to estimate its frequency
(in other cases, other notions of ``overlap'' can be considered such as edge
overlap, see \cite{calders11} for an overview). The number of occurrences also
has drawbacks from a statistical point of view, in the sense that occurrences of
patterns overlap and do not represent independent observations of the phenomenon
described by the pattern.

Earlier work, e.g., \cite{vanetik02} and \cite{calders11}, have considered this
problem from the point of view of pattern mining, and have considered several
combinations of matching operators (e.g., homomorphism, isomorphism,
homeomorphism) and overlap (e.g., vertex overlap, edge overlap). Calders et
al.\cite{calders11} have shown that for a large class of such settings, support
measures exist which are anti-monotonic and satisfy a number of common counting
intuitions. The maximal and minimal support measures can only be computed by
solving a maximal independent set or minimum clique partition problem, which is
NP hard in the number of occurrences. \cite{calders11} also showed a polynomial
time computable measure sandwiched between these two and based on the Lovasz
$\theta$ function. The frequency measure we consider in this paper, \emph{the
dependency weighted count} presented in Section~\ref{sec:dwc}, is a
generalization to databases of the $s$-measure introduced
in~\cite{wang_efficiently_2013}, where it is shown that $s$-measure satisfies
the nice properties introduced by \cite{calders11} and can be more efficiently
computed. They also argued that the measure makes more sense from a statistical
point of view, see also~\cite{WangPhD}.
% Wang, Yuyi. From Graph Patterns to Networked Statistics, PhD thesis, Informatics Section, Department of Computer Science, Faculty of Engineering Science, July 2015, Bruynooghe, Maurice and Ramon, Jan (supervisors) 

\paragraph{Conjunctive queries and factorized databases.} Conjunctive queries
are arguably one of the most studied classes of queries, covering a large body of
natural queries since they correspond to the SELECT-PROJECT-JOIN fragment of SQL
and have strong relations with the \emph{Constraint Satisfaction
  Problem}~\cite{Dechter} studied in AI. Given a conjunctive query $Q = S_1(X_1)
\wedge \dots \wedge S_k(X_k)$ with free variables $X
\subseteq \bigcup_{i=1}^k X_i$ (the others are existentially quantified)
and a database $\db$ on domain $D$, computing the answer set $Q(\db) \subseteq D^X$ of
$Q$ on database $\db$ is well-known to be $\NP$-complete~\cite{chandra77} when
both query and database are given as part of the input. A successful line of
research consists in finding classes of conjunctive queries that are
\emph{tractable}, that is, a class $C$ of conjunctive queries such that for
every $Q \in C$ and database $\db$, one can decide whether $Q(\db) \neq
\emptyset$ in polynomial time in the size of the $Q$ and $\db$. Yannakakis
initiated this research by showing in~\cite{Yannakakis} that so-called
\emph{$\alpha$-acyclic} queries can be solved in linear time in the size of the
database, opening the way to several
generalisations~\cite{GottlobLS01,CapelliDM14,grohe2014constraint,marx_tractable_2011}.

The idea underlying this body of work is that one can exploit the structure of
the interaction between variables and atoms to evaluate a conjunctive query
efficiently. This interaction is characterized by the hypergraph
$\mathcal{H}(Q)$ whose vertices are the variables $\varx$ of the query and edges
are the variables of its atoms, that is $\{X_i \mid 1 \leq i \leq k\}$ using above
notations. 
This hypergraph is then decomposed following a tree, in the same spirit
as what is done on graphs with tree decompositions. This decomposition is then
used to evaluate the query. The complexity of this evaluation depends on a
notion of width of the decomposition, that is, a rational number $k$ is
associated to the decomposition to measure its complexity. The smaller the
width, the better the algorithm performs. Several notions of width have been
introduced, such as, from the least to the most general one, hypertreewidth,
generalized hypertreewidth~\cite{gottlob_hypertree_2002} or fractional hypertree
width~\cite{grohe2014constraint} (see \cite{gottlob2016hypertree} for a survey),
all giving polynomial time algorithms for the query evaluation problem.

This approach has been shown to work to efficiently solve more involved
aggregation tasks on conjunctive queries such as
counting~\cite{pichler_tractable_2013,DurandM15} or
enumeration~\cite{bagan2007acyclic} and has found applications in practical
tools in order to design good query
plans~\cite{aberger2017emptyheaded,afrati2014gym}. More recently, Olteanu et
al.~\cite{olteanu2012factorised} proposed the framework of factorized databases,
unifying these approaches. 
\reviewer{4}{ \cite{olteanu2012factorised} discusses factorized representations for arbitrary conjunctive queries, not only for full conjunctive queries}
They have shown that when $Q$ has bounded (fractional
hypertree) width and is not existentially quantified, $Q(\db)$ can be efficiently 
represented by a \ddcircuit, i.e. a circuit performing Cartesian product and disjoint union, 
starting with atomic relations.
This representation is of size polynomial in the size of the database and the
query, which can be exponentially more succinct than the explicit list of
answers. This circuit representation allows to solve several aggregation
problems such as counting or probabilistic evaluation in time polynomial in the
\emph{size} of the representation. 
This two steps approach of first changing the
representation of the data before analysing it can be seen as a form of
knowledge compilation~\cite{darwiche_knowledge_nodate,olteanu2016factorized}, a
technique used in AI to solve various reasoning problems on complex data. From
this point of view, the factorized databases considered
in~\cite{olteanu2012factorised} exactly correspond to the class of circuits known
as structured decision DNNF~\cite{pipatsrisawat_new_nodate} in knowledge
compilation. In this paper, we consider a slight generalization of these objects
that we will call {\ddcircuit}s. These circuits correspond to the
so-called deterministic DNNF introduced by Darwiche
in~\cite{darwiche_decomposable_2001}.

\reviewer{4}{It is claimed that factorized databases correspond exactly to structured decision DNNF. However, \cite{olteanu2012factorised} does not state that. One difference is that the former are over multivalued variables and the latter over binary variables. Another reason has to do with the structure of a factorized database, which is defined by a d-tree that captured conditional independence in the data; this d-tree is more expressive than the v-tree of sd-DNNFs. Furthermore, sd-DNNFs may represent formulas that are not necessarily DNFs of clauses with the same arity (and typed variables).}

Factorized databases have already been used in the context of solving statistical
tasks on the data by Schleich et al.~\cite{schleich2016learning} where they show
that one can perform linear regression on data represented as a factorized
databases much more efficiently than by first enumerating the complete answer
set. We use a similar approach to solve our problem in this paper.

\reviewer{3}{in the Introduction the authors say that they will discuss the differences wrt. \cite{pichler_tractable_2013} in the related work. However, such a discussion is missing}

